Towards Practical Overlay Networks for Decentralized Federated Learning

Decentralized federated learning (DFL) uses peer-to-peer communication to avoid the single point of failure problem in federated learning and has been considered an attractive solution for machine learning tasks on distributed devices. We provide the first solution to a fundamental network problem of DFL: what overlay network should DFL use to achieve fast training of highly accurate models, low communication, and decentralized construction and maintenance? Overlay topologies of DFL have been investigated, but no existing DFL topology includes decentralized protocols for network construction and topology maintenance. Without these protocols, DFL cannot run in practice. This work presents an overlay network, called FedLay, which provides fast training and low communication cost for practical DFL. FedLay is the first solution for constructing near-random regular topologies in a decentralized manner and maintaining the topologies under node joins and failures. Experiments based on prototype implementation and simulations show that FedLay achieves the fastest model convergence and highest accuracy on real datasets compared to existing DFL solutions while incurring small communication costs and being resilient to node joins and failures.

==> 4.evaluation.tex <==
% 
%
%

\textbf{Environment settings.} To evaluate our design, we use 10 AWS EC2 with 4 GiB of RAM and 2GHz CPU. To expand the evaluation in large scale and more settings
we also use a desktop with graphics card to simulate the global training for cases which involve more than 50 clients. We evaluate the overall performance 
of our protocols with 3 different neural network models and datasets \ref{table:1}. 
\begin{table}[h!]
\begin{center}
    \begin{tabular}{ |c c c| } 
     \hline
     Dataset & Model & \# of Parameters\\ 
     \hline
     MNIST & MLP & ~250,000\\ 
     \hline
     CNN & CIFAR10 & ~5,100,000  \\ 
     \hline
     LSTM & Shakespeare & ~4,800,000 \\ 
     \hline
    \end{tabular}
\end{center}
\caption{Models and datasets we use to evaluate our protocol}
\label{table:1}
\end{table}

\subsection*{Flexibility}

\textbf{Flexible degree / single join / bulk join}

To gain the best trade off between degrees of graph topology and overall accuracy, we increasingly expand the dimensions of virtual coordinates of each node which means increase the degrees of the topology 
and construct the networking according to the topology we generates. 
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/degree-acc.pdf}
        \caption{We increase the degrees of each node by incrementing the dimensions of the virtual coordinate}
        \label{fig:da}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/degree-cost.pdf}
        \caption{We evaluate of cost-effective of adding degrees by comparing them with under the scope of the communication costs}
        \label{fig:dc}
    \end{subfigure}
       \caption{Accuracy vs degrees}
       \label{fig:degree}
\end{figure}
In the case of 100 nodes in total, a 10-degree graph is sufficiently to squeeze out the beneficial expander property of the graph and converge to its best effort.
Since most of the resources and time are spent on the training procedure, the cost of initialization process is negligible. We could see from the results\ref{fig:degree} that 
as the degree increases to over 8, the cost-effectiveness of adding more degrees tops. However, to reach the best overall accuracy, we could only sacrifice some
cost-effectiveness. 

To assess the performance, we compare our design to the vanilla federated learning and Gaia \cite{gaia} under the same communication budget and similar condition.
To make the Gaia be fully decentralized, we setup parameters server on each node and add as many nodes until it reach the same communication budget as our work.
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/method-acc.pdf}
        \caption{Global accuracy evaluated under MNIST and MLP}
        \label{fig:mehod1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/method-acc-cifar.pdf}
        \caption{Global accuracy evaluated under CIFAR10 and CNN}
        \label{fig:method2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/method-acc-shakes.pdf}
        \caption{Global accuracy evaluated under Shakespeare and LSTM}
        \label{fig:method3}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/nodes.pdf}
        \caption{Number of nodes participated in each round}
        \label{fig:method4}
    \end{subfigure}
       \caption{Accuracy \YF{data need to be corrected later.. (for Federated-L)}}
       \label{fig:method}
\end{figure}

From the result\ref{fig:method}, our approach has the best overall accuracy and stability. Since the vanilla federated learning can only pick a small fraction
of the clients in each global round, it is hard to reach a stable convergence under a communication budget and Non-IID data. Gaia has a good stability 
but it requires fully connected topology, so the number of the nodes that could participate\ref{fig:method4} in the whole training process is very limited.

Join protocol not only consists the construction of the networks, but also offers a flexible way to incrementally expand the network. Here, evaluate the 
process of a new node joining a training networks\ref{fig:join}. For a well-trained and stable networks, the performance of a joining node should be similar.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/join-acc.pdf}
    \caption{Bulk Joining node vs Global accuracy}
    \includegraphics[width=0.4\textwidth]{figure/join-single-acc.pdf}
    \caption{Single Joining node vs Global accuracy}
    \label{fig:join}
\end{figure}

From figure \ref{fig:join}, we can see out networks could quickly response to the incoming new nodes and take the joining node 

To simulate the real world scenarios where many users use similar devices and keep collecting and storing their own data and communicate through Internet with
different connection situations, we test the clients (end-users) will vary in local datasets and communication bandwidth. In our heterogeneous network settings, 
clients have similar computational power and the latency of the communication is trivial compared to the cost of transferring the updates of the models.

\subsection*{Against Non-iid data}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/label-heatmap.pdf}
    \caption{x-axis: clients with the label in its local dataset, y-axis: target label acc. To evaluate the performance of the non-iid settings. In the decentralized networks
    the client/node can correctly label the targets which are not in the local dataset}
    \label{fig:label-heatmap}
\end{figure}

The heatmap\ref{fig:label-heatmap} shows the inference accuracy of the alien labels. Although the local label tends to have a higher accuracy, the alien labels can also be evaluated correctly.




In practical, the data would not be well distributed for all sorts of training in general, so we first evaluate the performance of the IID vs. Non-IID distributions\ref{fig:id}. To make our evaluation 
closer to the real world applications, we conduct all the following experiments based on the Non-IID datasets. To create the Non-IID dataset, like most 
empirical work on synthetic non-IID datasets, we focused on label distribution skew, 
where a non-IID dataset is formed by partitioning a "flat" existing dataset based on the labels. 

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/dataset-acc.pdf}
    \caption{IID-MNIST vs Non-IID MNIST\textbf{could be substituted by heatmap figure???}}
    \label{fig:nid}
\end{figure}

We could see a heavy degradation on the overall accuracy on our system, as all the federated learning scheme mentioned in \cite{pmlr-v119-hsieh20a}. In the following 
evaluation, our work generalize against the Non-IID dataset because of the beneficial graph topology.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/cdf-sa-mnist.pdf}
    \caption{Simple Average in Non-IID MNIST test}
    \label{fig:cdf-sa-mnist}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/cdf-dc-mnist.pdf}
    \caption{Average with Data Divergence Confidence in Non-IID MNIST test}
    \label{fig:cdf-dc-mnist}
\end{figure}

This shows our performance when averaging weighted with Data Divergence Confidence in a Non-IID settings. 
We see from the \ref{fig:cdf-sa-mnist} that
although the network structure itself works against the Non-IID dataset efficiently,
 the performance could be boosted by using Data Divergence Confidence.



\subsection*{Asynchronous}

\textbf{Some figures to show the performance degradation in a Async situation: FedAvg and other works vs our work.}


Older implementation of asynchronous scenarios. 
The nodes still aggregate in a fixed time slots. The client will just drop certain percentile (asyncr)
of updates from the neighbors in order to catch the time.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/async-acc.pdf}
    \caption{Average with Data Divergence Confidence in Non-IID MNIST test}
    \label{fig:async-acc-mnist}
\end{figure}

New implementation of asynchronous scenarios. Each node could set its own pace of aggregation while timely serving their data to theri neighbors if requested.
To boost the performance, we use the speed of the aggregating as weights in the aggregating procedure. 

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/cdf-sa-mnist.pdf}
    \caption{Simple Average in Non-IID MNIST test}
    \label{fig:cdf-dc-mnist-1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figure/cdf-cc-mnist.pdf}
    \caption{Average with Communication Confidence in Non-IID MNIST test}
    \label{fig:cdf-cc-mnist}
\end{figure}
